A Self-Penalizing Objective Function for Scalable Interaction Detection

We tackle the problem of nonparametric variable selection with a focus on discovering interactions between variables. With $p$ variables there are $O(p^s)$ possible order-$s$ interactions making exhaustive search infeasible. It is nonetheless possible to identify the variables involved in interactions with only linear computation cost, $O(p)$. The trick is to maximize a class of parametrized nonparametric dependence measures which we call metric learning objectives; the landscape of these nonconvex objective functions is sensitive to interactions but the objectives themselves do not explicitly model interactions. Three properties make metric learning objectives highly attractive: (a) The stationary points of the objective are automatically sparse (i.e. performs selection) -- no explicit $\ell_1$ penalization is needed. (b) All stationary points of the objective exclude noise variables with high probability. (c) Guaranteed recovery of all signal variables without needing to reach the objective's global maxima or special stationary points. The second and third properties mean that all our theoretical results apply in the practical case where one uses gradient ascent to maximize the metric learning objective. While not all metric learning objectives enjoy good statistical power, we design an objective based on $\ell_1$ kernels that does exhibit favorable power: it recovers (i) main effects with $n \sim \log p$ samples, (ii) hierarchical interactions with $n \sim \log p$ samples and (iii) order-$s$ pure interactions with $n \sim p^{2(s-1)}\log p$ samples.

==> uniform_convergence.tex <==

\section{Uniform Convergence Results}
\label{sec:uniform-convergence}

%\rfcomment{I need to change the main result section below.}

\subsection{Main Results}
In this section, we study the uniform convergence of the empirical objective 
$F(\beta; \Q_n)$ to population objective $F(\beta; \Q)$ over the constraint 
set $\beta \in \mathcal{B}$, where we recall the definition
$\mathcal{B} = \left\{\beta \in \R_+^p: \norm{\beta}_1 \le b\right\}$. 
Here we restrict $\Q$ to be a reweighting distribution, i.e., $\Q = \Q^w$ for 
some nonnegative weight function $w$, where formally $\Q^w$ is defined as the unique 
probability measure that satisfies $dQ^w(x,y) \propto dP(x, y) \cdot w(x, y)$. 
It is helpful for the reader to keep in mind, for the purpose of studying metric learning algorithm, 
the underlying distribution $\Q$ of interest is the reweighting distribution 
$\Q= \Q^A (= \Q^{w_A})$ where $A \subseteq [p]$.

The rest of the section is organized as follows. 
\begin{itemize}
\item We start with a general result (Proposition~\ref{prop:finite-infinite-objective-gradient-bound}) 
	that establishes the uniform convergence of $F(\beta; \Q_n)$ to $F(\beta; \Q)$ for a generic 
	reweighting distribution $\Q = \Q^w$ that satisfies the assumption~\ref{assumption:F-w} (see below for the definition 
	of assumption~\ref{assumption:F-w}). We wish that assumption~\ref{assumption:F-w}
	clarifies the essential property for the distribution $\Q$ to satisfy 
	the uniform convergence guarantee. 
\item We next show in Proposition~\ref{proposition:weight_subset} that any reweighting distribution
	$\Q = \Q^A$ where $A \subseteq [p]$ satisfies the assumption~\ref{assumption:F-w}.
\item Finally, we combine the above results to establish the uniform convergence of 
	$F(\beta; \Q_n)$ to $F(\beta; \Q)$ for any reweighting distribution $\Q = \Q^A$. 
\end{itemize}

Here is the abstract assumption on the reweighting distribution $\Q$ that we need in order to establish the 
uniform convergence result. 

\renewcommand{\theassumption}{Q}

%\begin{assumption}
%\label{assumption:f-completely-monotone-general}
%That $f \in \mathcal{C}[0, \infty)$ satisfies $f^\prime$ is completely monotone. 
%\end{assumption}
\newcounter{saveassumption}
\setcounter{saveassumption}{\value{assumption}}

\begin{assumption}
\label{assumption:F-w}
Let $\Q = \Q^w$ be the (reweighting) distribution associated with some weight function 
$w(x,y)$. Assume the weight function $w$ satisfies
\begin{itemize}
\item The weight function is bounded: $0 \le w(X, Y) \le 1$ under $\P$. 
\item The class label is balanced after reweighting: 
	\begin{equation*}
		\Q(Y=0) = \Q(Y =1). 
	\end{equation*} 
\item For some constant $\varrho > 0$, we have that
\begin{equation*}
\begin{split}
	\popexpB[w(X, Y) w(X', Y')] &\ge \varrho^2,\\
	\popexpW[w(X, Y) w(X', Y')] &\ge \varrho^2.
\end{split}
\end{equation*}
	Here the expectation $\E$ is taken under measure $\P$. 
\end{itemize}
\end{assumption}

\paragraph{Notation}
We wish to emphasize that throughout the section, the notation $\E$ always stands for the expectation 
under the common probability measure $\P$ (and not under the probability measure $\Q$!). The 
reason is that we wish to state and prove our results under a common measure $\P$ so that we can easily relate 
results for different measures $\Q^\prime, \Q^{\prime\prime}, \ldots$. The way to denote the expectation under 
a reweighting disribution $\Q = \Q^w$ is to use the notation $\E^w$, where $w$ is the weight function associated
with $\Q$. 


%\begin{assumption}
%\label{assumption:X-bound}
%The covariate $X$ satisfies $|\diff|_\infty \le M$ almost surely. 
%\end{assumption}

\hspace{3cm}

Proposition~\ref{prop:finite-infinite-objective-gradient-bound} is the main result of the section, 
which establishes a uniform convergence result for a generic distribution $\Q$ satisfying 
assumption~\ref{assumption:F-w}. 


\setcounter{assumption}{0}
\renewcommand{\theassumption}{\arabic{assumption}}

\begin{proposition}
\label{prop:finite-infinite-objective-gradient-bound}
Assume Assumptions (A1)-(A2). Then we have for some constant $C > 0$ that depends only on 
$b, M, \varrho, f(0), f^\prime(0), f^{\prime\prime}(0)$ such that for any probability 
distribution $\Q$ satisfying Assumption~\ref{assumption:F-w}, we have 
\begin{enumerate}
\item For any $t > 0$, with probability at least $1-p^{-t^{2}} - e^{-n\varrho^2/32}$ under $\P$, 
	\begin{equation*}
	\begin{split}
		\sup_{\beta \in \mathcal{B}}
			\left|F(\beta; \Q_n) - F(\beta; \Q)\right|
				 \leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
	\end{split}
	\end{equation*}
\item For any $t > 0$, with probability at least $1-p^{-t^{2}} - e^{-n\varrho^2/32}$ under $\P$, 
	\begin{equation*}
	\begin{split}
		\sup_{j \in [p]} \sup_{\beta \in \mathcal{B}}
			\left|\frac{\partial}{\partial \beta_j} F(\beta; \Q_n) - 
				\frac{\partial}{\partial \beta_j} F(\beta; \Q)\right|
 					\leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
	\end{split}
	\end{equation*}
\end{enumerate}
\end{proposition}

\setcounter{assumption}{\value{saveassumption}}  % Set counters to
\renewcommand{\theassumption}{\arabic{assumption}}

Proposition~\ref{prop:finite-infinite-objective-gradient-bound} provides a uniform convergence 
result for a generic reweighting distribution $\Q$ that satisfies Assumption~\ref{assumption:F-w}. 
Below we study the uniform convergence for some specific choices of $\Q$. For any subset 
$A \subseteq [p]$, recall the reweighing distribution $\Q^A$ where $dQ^A(x, y) \propto dP(x, y) \cdot w_A(x, y)$
and where the weighting function $w_A$ is defined by 
\begin{equation*}
w_A(x, y) = 1 - \P(Y = y \mid X_A = x_A).
\end{equation*}   
Proposition~\ref{proposition:weight_subset} shows that the reweighting distribution $\Q^A$ 
satisfies~Assumption~\ref{assumption:F-w} under Assumption (A3). We defer the proof to 
Section~\ref{sec:proof-weight_subset}.
\begin{proposition}
\label{proposition:weight_subset}
Assume Assumption~(A3). Then for any set $A \subseteq [p]$, 
the reweighting function $w_{A}\left(x,y\right)=1 - \P\left(Y=y|X_{A}=x\right)$ satisfies
\begin{enumerate}
\item The weight function is bounded: $0 \le w_A(X, Y) \le 1$ under $\P$. 
\item The class label is balanced after reweighting: 
	\begin{equation*}
		\Q^A(Y = 0) = \Q^A(Y = 1) 
	\end{equation*} 
\item For the constant $\varrho > 0$ in the statement of Assumption (A3), we have
\begin{equation}
\label{eq:min_class_size}
\begin{split}
&\popexpB\left[w_{A}\left(X,Y\right)w_{A}\left(X',Y'\right)\right]  \ge  \varrho^2, ~~  \\
&\popexpW\left[w_{A}\left(X,Y\right)w_{A}\left(X',Y'\right)\right] \ge \varrho^{2}.
\end{split}
\end{equation}
\end{enumerate}
In above, the expectation $\E$ is taken under the probability measure $\P$. 
\end{proposition}

Proposition~\ref{prop:finite-infinite-objective-gradient-bound} and Proposition~\ref{proposition:weight_subset} 
immediately yield Corollary~\ref{cor:finite-infinite-objective-gradient-bound} below. 
\begin{corollary}
\label{cor:finite-infinite-objective-gradient-bound}
Assume Assumptions (A1)-(A3). There exists a constant $C > 0$ that depends only on 
$b, M, \varrho, f(0), f^\prime(0), f^{\prime\prime}(0)$ such that for any subset $A \subseteq [p]$, we have  
\begin{enumerate}
\item For any $t > 0$, with probability at least $1-p^{-t^{2}} - e^{-n\varrho^2/32}$ under $\P$, 
	\begin{equation*}
	\begin{split}
		\sup_{\beta \in \mathcal{B}}
			\left|F(\beta; \Q_n^A) - F(\beta; \Q^A)\right|
				 \leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
	\end{split}
	\end{equation*}
\item For any $t > 0$, with probability at least $1-p^{-t^{2}} - e^{-n\varrho^2/32}$ under $\P$, 
	\begin{equation*}
	\begin{split}
		\sup_{j \in [p]} \sup_{\beta \in \mathcal{B}}
			\left|\frac{\partial}{\partial \beta_j} F(\beta; \Q_n^A) - 
				\frac{\partial}{\partial \beta_j} F(\beta; \Q^A)\right|
 					\leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
	\end{split}
	\end{equation*}
\end{enumerate}
\end{corollary}


\subsection{Proof of Proposition~\ref{prop:finite-infinite-objective-gradient-bound}}
\label{sec:proof-finite-infinite-gradient-bound}
Let $\Q$ be any probability measure that satisfies Assumption~\ref{assumption:F-w}. 
Let $w(x, y) \propto \frac{dQ}{dP}(x, y)$ denote the weight function associated with $\Q$
so that $\Q = \Q^w$ and that weight function $w$ satisfies the conditions in the 
Assumption~\ref{assumption:F-w}.


To start with, we compute
\begin{equation*}
\begin{split}
	\left|F(\beta; \Q_n) - F(\beta; \Q)\right|
		&=  \left|(\empexpdiff^w - \popexpdiff^w)[f(\langle \beta, \diff\rangle)]\right|
	\\
	\left|\frac{\partial}{\partial \beta_j} F(\beta; \Q_n) -
			\frac{\partial}{\partial \beta_j} F(\beta; \Q) \right| 
	&= \left|(\empexpdiff^w - \popexpdiff^w)[\diff_j \cdot f^\prime(\langle \beta, \diff\rangle)]\right|
\end{split}	
\end{equation*}
By triangle inequality, we obtain
\begin{equation}
\label{eqn:prop-no-stationary-n-finite-bound}
\begin{split}
	\left|F(\beta; \Q_n) - F(\beta; \Q)\right|
		&\le \bar{\eps}_{n, B}(\beta) +  \bar{\eps}_{n, W}(\beta) \\
	\left|\frac{\partial}{\partial \beta_j} F(\beta; \Q_n) -
			\frac{\partial}{\partial \beta_j} F(\beta; \Q) \right| 
		&\le \eps_{n, B, j}(\beta) +  \eps_{n, W, j}(\beta)
\end{split}
\end{equation}
where we define the empirical deviations
\begin{equation}
\label{eqn:def-emp-dev}
\begin{split}
 \bar{\eps}_{n, B}(\beta)  &=  \left|(\empexpB^w - \popexpB^w)[f(\langle \beta, \diff\rangle)]\right| \\
 \bar{\eps}_{n, W}(\beta)  &=  \left|(\empexpW^w - \popexpW^w)[f(\langle \beta, \diff\rangle)]\right| \\
\eps_{n, B, j}\left(\beta\right)&=\left|(\empexpB^w - \popexpB^w)\left[\diff_j \cdot 
	f^\prime\left(\left\langle \beta,\diff\right\rangle \right)\right]\right|. \\
\eps_{n, W, j}\left(\beta\right)&=\left|(\empexpW^w - \popexpW^w)\left[\diff_j \cdot 
	f^\prime\left(\left\langle \beta,\diff\right\rangle \right)\right]\right|. 
\end{split}
\end{equation}

Following equation~\eqref{eqn:prop-no-stationary-n-finite-bound}, the key to the proof is to 
provide high probability upper bounds onto the following (random) quantities 
\begin{equation*}
	\sup_{\beta \in \mathcal{B}}  \bar{\eps}_{n, B}(\beta), ~~
	\sup_{\beta \in \mathcal{B}}  \bar{\eps}_{n, W}(\beta), ~~
	\sup_{j \in [p]}\sup_{\beta \in \mathcal{B}}  {\eps}_{n, B, j}(\beta), ~~
	\sup_{j \in [p]}\sup_{\beta \in \mathcal{B}}  {\eps}_{n, W, j}(\beta).
\end{equation*}
Lemma~\ref{lem:big_emp_dev} does this technical work, whose proof, which 
is based on the empirical process theory, is deferred to Section~\ref{sec:proof-lemma-big_emp_dev}.

\begin{lemma}
\label{lem:big_emp_dev}
Assume Assumptions~(A1)--(A2). Assume $w(x, y)$ satisfies
\begin{itemize}
\item The weight function is $0 \le w(X, Y) \le 1$. 
\item For some constant $\varrho > 0$, we have that 
\begin{equation*}
\begin{split}
	\popexpB[w(X, Y) w(X', Y')] &\ge \varrho^2,\\
	\popexpW[w(X, Y) w(X', Y')] &\ge \varrho^2.
\end{split}
\end{equation*} 
\end{itemize} 
Let $g, h$ be two functions that satisfy 
\begin{itemize}
\item $x \mapsto g(x)$ is Lipschitz with Lipschitz constant $L$. 
\item $x \mapsto |g(x)|$ is upper bounded by $G$ for all $x \in [0, 2Mb]$.
\item $x \mapsto |h(x)|$ is upper bounded by $H$ for all $x \in [0, M]$. 
\end{itemize}
Consider the two random functions:  
\begin{equation}
\begin{split}
\delta_{n, W, j}(\beta) &= 
	\left|(\empexpW^w - \popexpW^w)\left[g(\langle \beta, \diff \rangle) \cdot h(\diff_j)\right]\right| \\
\delta_{n, B, j}(\beta) &= 
	\left|(\empexpW^w - \popexpW^w)\left[g(\langle \beta, \diff \rangle) \cdot h(\diff_j)\right]\right|
\end{split}
\end{equation}
There exists some constant $C > 0$ that depends only on 
$G, H, L, b, M,\varrho$ such that we have with probability at least $1-p^{-t^{2}}-e^{-n\varrho^2/32}$, 
\begin{equation}
\begin{split}
	\sup_{\beta \in \mathcal{B}} \left(\delta_{n, B, j}\left(\beta\right) 
		+ \delta_{n, W, j}\left(\beta\right)\right)
			 \leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
\end{split}
\end{equation}
%In above, $C > 0$ is a constant depending only on $b, M, \varrho, L, g(0)$.
\end{lemma}
We apply Lemma~\ref{lem:big_emp_dev} to two specific groups of choice of $(g, h)$. 
\begin{itemize}
\item We first specify $g(x) = f(x)$ and $h(x) \equiv 1$. Note that 	
 	$f$ is $f^\prime(0)$ Lipschitz since $f^\prime$ is completely monotone. Lemma
	\ref{lem:big_emp_dev} implies with probability at least $1-p^{-t^{2}}-e^{-n\varrho^2/32}$ under 
	$\P$, 
	\begin{equation*}
		\sup_{\beta \in \mathcal{B}} \left(\bar{\eps}_{n, B}\left(\beta\right) + \bar{\eps}_{n, W}\left(\beta\right)\right)
 			\leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t),
	\end{equation*}
	where $C > 0$ is a constant that depends only on $b, M, \varrho, f(0), f^\prime(0)$.
\item We next specify $g(x) = f^\prime(x)$ and $h(x) = x$. Note that 	
 	$f^\prime$ is $|f^{\prime\prime}(0)|$ Lipschitz since $f^\prime$ is completely monotone. Lemma
	\ref{lem:big_emp_dev} implies with probability at least $1-p^{-t^{2}}-e^{-n\varrho^2/32}$ under 
	$\P$, 
	\begin{equation*}
		\sup_{j \in [p]}\sup_{\beta \in \mathcal{B}} \left({\eps}_{n, B, j}\left(\beta\right) + {\eps}_{n, W, j}
			\left(\beta\right)\right) \leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
	\end{equation*}
	where $C > 0$ is a constant that depends only on $b, M, \varrho, f^\prime(0), f^{\prime\prime}(0)$.
\end{itemize}
Proposition~\ref{prop:finite-infinite-objective-gradient-bound} now follows straightforwardly from the previous 
discussions. 
%implies with probability at least $1-p^{-t^{2}}-e^{-n\varrho^2/32}$, 
%\begin{equation*}
%\begin{split}
%\sup_{j \in [p]} \sup_{\beta \in \mathcal{B}}
%\left|\frac{\partial}{\partial \beta_j} \ell_n(\beta; \lambda, w) - \frac{\partial}{\partial \beta_j} \ell_\infty(\beta; \lambda, w)\right|
% \leq C \cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
%\end{split}
%\end{equation*}
%This completes the proof of Proposition~\ref{prop:finite-infinite-gradient-bound}.



\subsubsection{Proof of Lemma~\ref{lem:big_emp_dev}}
\label{sec:proof-lemma-big_emp_dev}
For simplicity, we slightly modify the definition of the empirical 
average $\empexpB^w$ and $\empexpW^w$ in the proof below. 
Concretely, we define for any function $h(x, x', y, y')$
\begin{equation}
\begin{split}
\empexpB[h(X, X', Y, Y')] &=
	\frac{ \sum_{i \neq i'} w(X_i, Y_i) w(X_{i^\prime}, Y_{i^\prime})
	 	h(X_i, X_{i^\prime}, Y_i, Y_{i^\prime}) \mathbf{1}_{Y_i \neq Y_{i^\prime}}} 
	{\sum_{i \neq i'} w(X_i, Y_i) w(X_{i^\prime}, Y_{i^\prime})\mathbf{1}_{Y_i \neq Y_{i^\prime}}} \\
\empexpW[h(X, X', Y, Y')] &=
	 \frac{ \sum_{i \neq i'} w(X_i, Y_i) w(X_{i^\prime}, Y_{i^\prime})
	 	h(X_i, X_{i^\prime}, Y_i, Y_{i^\prime}) \mathbf{1}_{Y_i = Y_{i^\prime}}} 
	{\sum_{i \neq i'} w(X_i, Y_i) w(X_{i^\prime}, Y_{i^\prime})\mathbf{1}_{Y_i = Y_{i^\prime}}}.
\end{split}
\end{equation}
The only difference between the new definition above and the original definition in the main text is that, 
while the original definition sums over all possible tuples $(i, i')$ on the RHS where $1\le i, i' \le n$, 
the new definition only sums over all possible \emph{distinct} tuple $(i, i')$ where $1\le i, i' \le n$ and 
$i \neq i'$. One important claim is that such modification doesn't change qualitatively the uniform 
convergence result (and it can only change the numerical constants in the high probability bound). 
The reason why this is true is largely due to the fact that the weight $w(x, y)$ and the 
function $h(x, x', y, y') = g(\langle \beta, \diff \rangle) \cdot h(\diff_j)$ of interest is 
bounded---$0\le w(x, y) \le 1$ and $|h(x, x', y, y')| \le GH$ by assumption---so summing over all tuples $(i, i')$ versus
summing over all \emph{distinct} tuples $(i, i')$ do not make a real difference. The formal 
proof of this claim is tedious (simple, lengthy, but not insightful) and thus omitted. 

In the proof below, we will work under this definition of 
$\empexpB^w$ and $\empexpW^w$, and still the random quantities of interest are defined by 
\begin{equation}
\begin{split}
\delta_{n, W, j}(\beta) &= 
	\left|(\empexpW^w - \popexpW^w)\left[g(\langle \beta, \diff \rangle) \cdot h(\diff_j)\right]\right| \\
\delta_{n, B, j}(\beta) &= 
	\left|(\empexpW^w - \popexpW^w)\left[g(\langle \beta, \diff \rangle) \cdot h(\diff_j)\right]\right|
\end{split}
\end{equation}
We prove for any fixed $j \in [p]$, with probability at least 
$1-p^{-t^{2}} - e^{-n\varrho^2/32}$, %the bound on $\eps_{n, B, j}(\beta)$ 
\begin{equation}
\label{eqn:hig-prob-varepsilon-B}
\begin{split}
\sup_{\beta \in \mathcal{B}}~\delta_{n, B, j}(\beta) \leq C\cdot\sqrt{\frac{\log p}{n}} \cdot (1+t).
\end{split}
\end{equation}
holds for some large constant $C > 0$ depending on $G, H, L, b, M, \varrho$. An analogous 
high probability bound also holds for $\delta_{n, W, j}(\beta)$. Together, with a union bound, 
this proves Lemma~\ref{lem:big_emp_dev} as desired. 

Now we show equation~\eqref{eqn:hig-prob-varepsilon-B} holds with probability at least $1-p^{-t^{2}} - e^{-n\varrho^2/32}$. 
Fix $j \in [p]$. We introduce notational shorthand to simplify the proof below. We use $Z_i = (X_i, Y_i)$ to denote 
the i.i.d data pair. Introduce 
\begin{equation*}
\begin{split}
r_{\beta}(z_i, z_i') &= g\left(\langle \beta, \diff\rangle\right) \cdot h(\diff_j) \\
w(z_i, z_i') &= 1_{y_{i}\neq y_{i'}}w (z_i)w (z_{i'}) \\
q_\beta(z_i, z_i') &= r_\beta(z_i, z_i') w(z_i, z_i')
\end{split}	
\end{equation*}
where $w(z_i)$ is the weight. Let $\hat{\E}_n$ denote the empirical average over all the $n(n-1)$ 
distinct tuples $(i_1, i_2)$. By definition of $\empexpB^w, \popexpB^w$, 
\begin{equation*}
\empexpB^w[h_{\beta}(z, z')] = \frac{\hat{\E}_n  [q_{\beta}(z, z')]}{\hat{\E}_n [w(z, z')]}
	~~\text{and}~~
\popexpB^w[h_\beta(z, z')] = \frac{\E  [q_{\beta}(z, z')]}{\E [w(z, z')]}.
\end{equation*}
Hence, we have the identity 
\begin{equation}
\label{eqn:T-reexpress}
\sup_{\beta \in \mathcal{B}} \delta_{n, B, j}(\beta)= \sup_{\beta \in \mathcal{B}}
	\left|\frac{\hat{\E}_n  [q_{\beta}(z, z')]}{\hat{\E}_n [w(z, z')]} - \frac{\E  [q_{\beta}(z, z')]}{\E [w(z, z')]}\right|.
\end{equation}
Now we use the elementary inequality: for $a, a', b, b' \in \R$, 
\begin{equation*}
\left|\frac{b}{a} - \frac{b'}{a'}\right| \le \frac{1}{|aa'|} \left(|a-a'||b'| + |b-b'||a'|\right)
\end{equation*}
Applying this inequality to equation~\eqref{eqn:T-reexpress}, we obtain the bound
\begin{equation}
\label{eqn:a-first-bound-on-T}
\sup_{\beta \in \mathcal{B}} \delta_{n, B, j}(\beta) \le \frac{1}{\Gamma_n} \left(\Delta_{1, n} + \Delta_{2, n}\right) 
\end{equation}
where 
\begin{equation*}
\begin{split}
\Gamma_n &= \hat{\E}_n [w(z, z')] \cdot \E [w(z, z')] \\
\Delta_{1, n}& = \E [w(z, z')] \cdot \sup_{\beta \in \mathcal{B}}
		\left|(\hat{\E}_n  - \E) [q_{\beta}(z, z')]\right| \\
\Delta_{2, n} &= \left|(\hat{\E}_n  - \E) [w(z, z')]\right|\cdot
			\sup_{\beta \in \mathcal{B}} \E [q_\beta(z, z')]
\end{split}
\end{equation*}
To obtain high probability upper bound on $\sup_{\beta \in \mathcal{B}} \delta_{n, B, j}(\beta)$, it suffices 
to derive a high probability lower bound on $\Gamma_n$ and upper bound on $\Delta_{1, n}, \Delta_{2. n}$.
The following three technical lemma are useful towards this end. 


%\begin{lemma}
%\label{lemma:population-lower-bound-sample-size}
%The lower bound holds
%\begin{equation*}
%\E[w(z, z')] \ge \varrho^2. 
%\end{equation*}
%\end{lemma}
%Lemma~\ref{lemma:population-lower-bound-sample-size} is a special case of
%Lemma~\ref{proposition:weight_subset}, whose proof can be found in 


\begin{lemma}
\label{lemma:w-concentration}
We have with probability at least $1-e^{-4t^2}$: 
\begin{equation*}
\left|(\hat{\E}_n  - \E) [w(z, z')]\right| \le \sqrt{\frac{1}{n}} \cdot t. 
\end{equation*}
\end{lemma}
\begin{proof}
Note that the weights $0 \le w\le 1$ by assumption. The lemma is a consequence of Hoeffding's 
inequality for U-statistics (see Lemma~\ref{lemma:Hoeffding}).
\end{proof}


\begin{lemma}
\label{lemma:w-lower-bound-concentration}
We have with probability at least $1-e^{-n \varrho^2/32}$: 
\begin{equation*}
\hat{\E}_n [w(z, z')] \ge \half \varrho.  
\end{equation*}
\end{lemma}
\begin{proof}
By assumption, $0 \le w \le 1$ and $\E[w(z, z')] \ge \varrho$. The lemma is a 
consequence of Bernstein's inequality for U-statistics (see Lemma~\ref{lemma:Hoeffding}). 
\end{proof}


\begin{lemma}
\label{lemma:bound-on-q-beta}
For any $\beta \in \mathcal{B}$, we have 
\begin{equation*}
\sup_{z, z'} \left|q_\beta(z, z')\right| \le GH.
\end{equation*}
\end{lemma}
\begin{proof}
Assumption~(A2) gives $0 \le \diffj \le 2M$ for all $j \in [p]$, 
and moreover gives $0\le \langle \beta, \diff\rangle \le 2Mb$ 
for all $\beta \in \mathcal{B}$ by H\"{o}lder's inequality. 
Assumption~\ref{assumption:F-w} gives $0\le w\le 1$.   
Thus, we have for all $\beta\in \mathcal{B}$,
\begin{equation*}
\sup_{z, z'} |q_\beta(z, z')| \le GH.
\end{equation*}
This completes the proof of Lemma~\ref{lemma:bound-on-q-beta}. 
\end{proof}

\begin{lemma}
\label{lemma:high-prob-Q}
We have with probability at least $1-p^{-t^2}$: 
\begin{equation*}
\sup_{\beta \in \mathcal{B}}
		\left|(\hat{\E}_n  - \E) [q_{\beta}(z, z')]\right| \le C\sqrt{\frac{\log p}{n}} \cdot (1+t). 
\end{equation*}
In above $C$ is a constant depending only on $b, M, L, G, H$.
\end{lemma}
We provide the proof of Lemma~\ref{lemma:high-prob-Q} into Section~\ref{sec:proof-lemma-high-prob-Q}.

Now we give high probability upper bound on 
$\sup_{\beta \in \mathcal{B}} \delta_{n, B, j}(\beta)$ using equation~\eqref{eqn:a-first-bound-on-T}. 
By Lemma~\ref{lemma:w-concentration}, Lemma~\ref{lemma:bound-on-q-beta} and 
Lemma~\ref{lemma:high-prob-Q}, the bound below
\begin{equation*}
\Delta_{1, n} \le C\cdot \sqrt{\frac{\log p}{n}} \cdot (1+t), ~~
\Delta_{2, n} \le C\cdot \sqrt{\frac{\log p}{n}}t
\end{equation*}
 holds with probability at least $1-2p^{-t^2}$, where $C > 0$ is some constant depending only on 
 $b, M, L, G, H$. Recall Assumption~\ref{assumption:F-w}: $\E [w(z, z')] \ge \varrho^2$. Thus
Lemma~\ref{lemma:w-lower-bound-concentration} further implies 
\begin{equation*}
\Gamma_n \ge \E [w(z, z')] \cdot \hat{\E}_n [w(z, z')] \ge \half \varrho^4.
\end{equation*}
with probability at least $1-e^{-n\varrho^2/32}$. Substitute the high probability bounds into 
equation~\eqref{eqn:a-first-bound-on-T}. We get with probability at least $1-2p^{-t^2} - e^{-n\varrho^2/32}$,
\begin{equation*}
\sup_{\beta \in \mathcal{B}} \delta_{n, B, j}(\beta) \le C\cdot \sqrt{\frac{\log p}{n}} \cdot (1+t).
\end{equation*}
where $C > 0$ is a constant that depends on  $b, M, \varrho, L, G, H$. This completes
the proof of Lemma~\ref{lem:big_emp_dev}.









%\section{Properties on Rebalancing Weights}
%\label{sec:balance_proofs}


%Therefore, A6 implies 
%\begin{equation*}
%\popexpB\left[w\left(X,Y\right)w\left(X',Y'\right)\right]\geq\varrho^{2}\qquad\popexpW\left[w\left(X,Y\right)w\left(X',Y'\right)\right]\geq\varrho^{2}.
%\end{equation*}



\subsubsection{Proof of Lemma~\ref{lemma:high-prob-Q}}
\label{sec:proof-lemma-high-prob-Q}
Let's denote the random variable
\begin{equation*}
W = \sup_{\beta \in \mathcal{B}}
		\left|(\hat{\E}_n  - \E) [q_{\beta}(z, z')]\right|.
\end{equation*}
We view $W\equiv W(Z_{1:n})$ as a function of the i.i.d data pair $Z_i = (X_i, Y_i)$. 
Lemma~\ref{lemma:bound-on-q-beta} implies that this function is of bounded difference 
with bound $2GH/n$, i.e., for any $Z_{1:n}$ and $Z^\prime_{1:n}$ differing in only 
one coordinate, 
\begin{equation*}
	\left|W(Z_{1:n}) - W(Z^\prime_{1:n})\right| \le \frac{2GH}{n}.
\end{equation*}
Thus, McDiarmid's bounded difference inequality \cite{Mcdiarmid89} gives
\begin{equation}
\label{eqn:Q-concentration}
W \leq \E[W]+2GH \cdot \sqrt{\frac{\log p}{n}} \cdot t
\end{equation}
holds with probability at least $1-p^{-t^{2}}$.

Now, we bound $\E[W]$. On a high level, our idea works as follows: viewing $W$ as the suprema of some 
empirical process, we symmetrize $W$ and bound the resulting Rademacher complexity with the
Ledoux-Talagrand contraction inequality~\cite{Ledoux13}. Formally, we decompose 
\begin{equation*}
q_\beta(z, z') = \phi\left(\langle \beta, \diff\rangle, z, z'\right) + \bar{\phi}\left(z, z'\right),
\end{equation*}
where $(z, z') \mapsto \bar{\phi}(z, z')$ and $(u, z, z') \mapsto \phi(u, z, z')$ are defined by 
\begin{equation*}
\begin{split}
	\bar{\phi}\left(z, z'\right) &= w(z, z') \cdot g(0) \cdot h(\diff_j)\\
	\phi(u, z, z') &= w(z, z') \cdot (g(u) - g(0)) \cdot h(\diff_j).
\end{split}
\end{equation*}
%Thus, we have the identity: 
We emphasize that the definition of the two functions $\phi$ and $\bar{\phi}$ are independent of 
$\beta \in \mathcal{B}$. By triangle inequality, we can upper bound 
\begin{equation}
\label{eqn:Q-Q'-bar-Q}
	\E[W] \le \E[W_1] + \E[W_2]
\end{equation}
where $W_1$ and $W_2$ are the supremum of some empirical process: 
\begin{equation*}
\begin{split}
	W_1 = \left|(\hat{\E}_n  - \E) [\bar{\phi}(z, z')]\right|~~\text{and}~~
	W_2 = \sup_{\beta \in \mathcal{B}}\left|(\hat{\E}_n  - \E) [\phi(\langle \beta, \diff\rangle, z, z')]\right|.
\end{split}
\end{equation*}
Below we bound $\E[W_1]$ and $\E[W_2]$ separately. Our major technique is to use symmetrization 
argument followed by Hoeffding~\cite{Hoeffding94} and Ledoux-Talagrand contraction
inequality~\cite{Ledoux13}. As both $W_1$ and $W_2$ involve averages of \emph{dependent} random variables, 
standard symmetrization argument does not immediately apply, for which reason we adapt a decoupling 
technique that is due to \citet{Hoeffding94} to overcome this technical difficulty. We introduce the notation. 
\begin{itemize}
\item Let $\sigma_{i,i'}$ be independent Rademacher random variables. 
\item Let $\bar{\phi}_{(i, i')} = \bar{\phi}\left(z_i, z_i'\right)$ and $\phi_{(i, i')}(u) = \phi\left(u, z_i, z_i'\right)$.
\item Let $\mathcal{I} = \left\{(i, i') \mid i \neq i', 1\le i, i' \le n\right\}$. A simple combinatorial argument shows that 
	we can decompose $\mathcal{I} = \cup_{j=1}^I \mathcal{I}_j$ where $I \le n$, $|\mathcal{I}_j| \ge \floor{\frac{n}{2}}$,  
	and where for any two different tuples $(i_1, i_2), (i_3, i_4) \in \mathcal{I}_j$ where $j \in [I]$, we have $i_k \neq i_l$ for 
	$1\le k < l \le 4$. For each $j \in [I]$, let $\hat{\E}_{n, j}$ denote the empirical average over the distinct tuples 
	$(i_1, i_2) \in \mathcal{I}_j$.
\end{itemize}

\paragraph{Part 1: Bound on $\E[W_1]$}
As $\mathcal{I} = \cup_{j=1}^I \mathcal{I}_j$, we have by triangle inequality 
%By triangle inequality, we can easily derive 
\begin{equation}
\label{eqn:Q-1-first-step}
\begin{split}
\E[W_1] \le \frac{1}{I} \sum_{j=1}^I \E \left[ \big|(\hat{\E}_{n, j}  - \E) [\bar{\phi}(z, z')]\big|\right] \le 
\max_{j \in [I]} \E \left[ \big|(\hat{\E}_{n, j}  - \E) [\bar{\phi}(z, z')]\big|\right]
\end{split}
\end{equation}
Now for each $j \in [I]$, $\hat{\E}_{n, j}[\bar{\phi}(z, z')]$ is the average of independent random variables. 
Invoking the standard symmetrization argument, we obtain 
\begin{equation}
\label{eqn:bound-Q-1-symmetrization}
\E[W_1] \le 2 \max_{j \in [I]} \E\left\{ \E_\sigma \bigg[\frac{1}{|\mathcal{I}_j|} \Big|\sum_{(i, i') \in \mathcal{I}_j} 
	\sigma_{i, i'} \bar{\phi}_{i, i'}\Big|\mid Z\bigg]\right\}.
\end{equation}
Note then $\sup_{i, i'}|\bar{\phi}_{i, i'}| \le GH$ since we have by assumption 
$0 \le w(z, z') \le 1$, $|g(0)| \le G$ and $\sup_{x \in [0, M]} |h(x)| \le H$.
As $\{\sigma_{i, i^\prime}\}_{i \neq i^\prime}$ are independent $1$-subgaussian random variables, we 
obtain the bound for all $j$: 
\begin{equation}
\label{eqn:bound-Q-1-main}
	 \E_\sigma \bigg[\frac{1}{|\mathcal{I}_j|} \Big|\sum_{i \neq i'} \sigma_{i, i'} \bar{\phi}_{i, i'}\Big|\mid Z\bigg] 
	 	\le GH \cdot \sqrt{\frac{1}{|\mathcal{I}_j|}} \le 2 GH \cdot \sqrt{\frac{1}{n}}.
\end{equation}
Substituting equation~\eqref{eqn:bound-Q-1-main} into equation~\eqref{eqn:bound-Q-1-symmetrization} 
yields the final bound 
\begin{equation}
\label{eqn:bar-Q-bound}
	\E[W_1] \le 4 GH \cdot \sqrt{\frac{1}{n}}.
\end{equation}

\paragraph{Part 2: Bound on $\E[W_2]$}
Similar to equation~\eqref{eqn:Q-1-first-step}, we have %by triangle inequality 
\begin{equation*}
\begin{split}
\E[W_2] \le \max_{j \in [I]} 
	\sup_{\beta \in \mathcal{B}}\left|(\hat{\E}_{n, j}  - \E) [\phi(\langle \beta, \diff\rangle, z, z')]\right|.
\end{split}
\end{equation*}
Now for each $j \in I$, $\hat{\E}_{n, j}[\phi(\langle \beta, \diff\rangle, z, z')]$ is the average of independent random variables. 
Invoking the standard symmetrization argument, we obtain 
\begin{equation}
\label{eqn:wtilde-T-one}
\E[W_2] \le 2 \max_{j \in [I]}\E\left\{ 
\mathbb{E}_{\sigma}\left[\sup_{\beta \in \mathcal{B}}
	\bigg|\frac{1}{|\mathcal{I}_j|}
		\sum_{(i, i') \in \mathcal{I}_j}\sigma_{i,i'}\cdot\phi_{i,i'}\left(\left\langle \beta, \diff\right\rangle \right) \bigg|\vert Z\right] \right\}.
%\E_\sigma \Big[\sup_{\beta \in \mathcal{B}}\frac{1}{n(n-1)} \Big|\sum_{i \neq i'} \sigma_{i, i'} {\phi}_{i, i'}(\langle \beta, \diff\rangle)\Big|\mid Z\Big]\right\}
\end{equation}
The inner expectation is over $\sigma_{i,i'}$ with the data $Z$ (all data $z_i$) fixed while the outer expectation is 
over $Z$. Now for any fixed $z_i, z_i'$, since we have 
\begin{equation*}
\begin{split}
\left|\frac{d}{du} \phi(u, z_i, z_i')\right| &= \left|w(z_i, z_i') \cdot h(\diff_j) \cdot g^\prime(u)\right| \le LH.
\end{split}
\end{equation*}
the mapping $u \to \phi_{i, i'}(\cdot, z_i, z_i')$ is Lipschitz with constant $LH$. Note further that 
$\phi_{i, i'}(0, z_i, z_i') = 0$. Hence, conditional on $\diff$, we may apply the Ledoux-Talagrand 
contraction~\cite{Ledoux13} inequality to obtain the following upper bound 
\begin{equation}
\label{eqn:wtilde-T-two}
\begin{split}
&\mathbb{E}_{\sigma}\left[\sup_{\beta \in \mathcal{B}}
	\bigg|\frac{1}{|\mathcal{I}_j|}
		\sum_{(i, i') \in \mathcal{I}_j}\sigma_{i,i'}\cdot\phi_{i,i'}\left(\left\langle \beta, \diff\right\rangle \right) \bigg|\vert Z\right] \\
& \leq2LH\cdot\mathbb{E}_{\sigma}\left[\sup_{\beta \in \mathcal{B}}
	\bigg|\frac{1}{|\mathcal{I}_j|} \sum_{(i, i') \in \mathcal{I}_j}\sigma_{i,i'}\left\langle \beta, \diff\right\rangle \bigg|\vert Z\right].
\end{split}
\end{equation}
To further bound the RHS, we notice the two key facts 
\begin{itemize}
\item $\{\sigma_{i, i^\prime}\}_{i \neq i^\prime}$ are mutually independent $1$-subgaussian random variables.
\item The $\ell_\infty$ bound on $\norm{\diff}_{\infty} \le M$ which is due to Assumption~(A2). 
\end{itemize}
Using the above facts, we can easily obtain the further bound 
\begin{equation}
\label{eqn:wtilde-T-three}
\begin{split}
&\mathbb{E}_{\sigma}\left[\sup_{\beta\in \mathcal{B}}
	\bigg|\frac{1}{|\mathcal{I}_j|} \sum_{(i, i') \in \mathcal{I}_j}\sigma_{i,i'}\left\langle \beta,\diff\right\rangle \bigg|\vert Z\right] \\
 & = 
 \mathbb{E}_{\sigma}\left[\sup_{\beta \in \R_+^{p}: \normsmall{\beta}_1 \le b}
 	\bigg|\Big\langle \beta, \frac{1}{|\mathcal{I}_j|} \sum_{(i, i') \in \mathcal{I}_j}\sigma_{i,i'}\diff\Big\rangle \bigg|\vert Z\right]\\
 &= b \cdot \mathbb{E}_{\sigma}\left[\bigg|\frac{1}{|\mathcal{I}_j|} \sum_{(i, i') \in \mathcal{I}_j}\sigma_{i,i'} \cdot \diff\bigg|_{\infty}\vert\diff\right]
 \le 2Mb \sqrt{\frac{\log p}{|\mathcal{I}_j|}}, %\le 22Mb \sqrt{\frac{\log p}{n}},
\end{split}
\end{equation}
Consequently, equations~\eqref{eqn:wtilde-T-one}--\eqref{eqn:wtilde-T-three} yield the final bound
\begin{equation}
\label{eqn:Q'-bound}
\E[W_2] \le 4MbLH \cdot \sqrt{\frac{\log p}{n}}.
\end{equation}

\paragraph{Summary}
Back to equation~\eqref{eqn:Q-concentration}. We use equations~\eqref{eqn:Q-Q'-bar-Q}, 
\eqref{eqn:bar-Q-bound} and~\eqref{eqn:Q'-bound} to conclude the following:  for any $t > 0$, 
with probability at least $1-p^{-t^2}$.
\begin{equation}
	Q \leq  8(2MbLH + GH) \cdot \sqrt{\frac{\log p}{n}} \cdot (1+t)
\label{eq:dev_fixed}
\end{equation}







%\subsection{XXX}
%
%\begin{lemma}
%\label{proposition:weight_subset}
%Assume Assumption (A5). Then for any set $A$, 
%the weight function $w_{A}\left(x,y\right)=P\left(Y=1-y|X_{A}=x\right)$ satisfies
% % and $Y \mid X = Y \mid X_S$. Then %for all $A \subseteq S$, 
%\begin{equation}
%\label{eq:min_class_size}
%\begin{split}
%&\popexpB\left[w_{A}\left(X,Y\right)w_{A}\left(X',Y'\right)\right]  \ge  \varrho^2, ~~  \\
%&\popexpW\left[w_{A}\left(X,Y\right)w_{A}\left(X',Y'\right)\right] \ge \varrho^{2}.
%\end{split}
%\end{equation}
%\end{lemma}
%We defer the proof of Lemma~\ref{proposition:weight_subset} in Section~\ref{sec:proof-weight_subset}. As an 
%immediate consequence, Lemma~\ref{proposition:weight_subset} implies the lower bound
%\begin{equation}
%\label{eqn:pop-lower-bound-ess}
%\E[w(z, z')] \ge \varrho^2. 
%\end{equation}


\subsection{Proof of Proposition \ref{proposition:weight_subset}}
\label{sec:proof-weight_subset}
The first part of Proposition~\ref{proposition:weight_subset} is trivial. The second 
part of Proposition~\ref{proposition:weight_subset} follows from the identity 
\begin{equation*}
\Q^A(Y = 1) = \E[w_A(X, 1) w_A(X, 0))] = \Q^A(Y = 0), 
\end{equation*}
and this identity can be proven easily by using the law of iterated expectation. 
Below, we prove the third part of Proposition~\ref{proposition:weight_subset}. 
That is, under Assumption (A3), we have equation~\eqref{eq:min_class_size} holds. 

Write $\pi(X_A) = \P(Y = 1 \mid X_A)$. Recall that $Y \mid X = Y \mid X_S$.
The proof is based on a fundamental inequality that holds for any set $A$: 
\begin{equation}
\label{eqn:weight-subset-one}
\E [\pi(X_A) \mid Y = 0] \ge \E[\pi(X_S) \mid Y = 0]. 
\end{equation}
To obtain this result, we note first for any set $A$: 
\begin{equation}
\label{eqn:weight-subset-one-one}
\begin{split}
\E [\pi(X_A) \mid Y = 0] &= \frac{1}{\P(Y = 0)} \E[\pi(X_A) \one_{Y= 0}] \\
			&= \frac{1}{\P(Y = 0)} \E[\pi(X_A) (1- \pi(X_A))] \\
			&= \frac{1}{\P(Y = 0)} \E[\Var(Y \mid X_A)].
\end{split}
\end{equation}
Next, for any set $A$, we have 
\begin{equation}
\label{eqn:weight-subset-one-two}
\Var(Y \mid X_A) \ge \E[\Var(Y \mid X_{S \cup (A\backslash S)}) \mid X_A] = \E[\Var(Y \mid X_S) \mid X_A].
\end{equation}
where the inequality follows from the conditional variance decomposition and the equality from
$Y|X = Y|X_{S}$. 
Substituting it into equation~\eqref{eqn:weight-subset-one-one}, we obtain the desired inequality~\eqref{eqn:weight-subset-one}
\begin{equation*}
\begin{split}
\E [\pi(X_A) \mid Y = 0] &= \frac{1}{\P(Y = 0)} \E[\Var(Y \mid X_A)] \\
	&\ge \frac{1}{\P(Y = 0)} \E[\Var(Y \mid X_S)] = \E [\pi(X_S) \mid Y = 0]
\end{split}
\end{equation*}

In the same way, one can show for any set $A$,
\begin{equation*}
\label{eqn:weight-subset-two}
\E[(1-\pi(X_A)) \mid Y = 1] \ge \E[(1-\pi(X_S)) \mid Y = 1]
\end{equation*}
%Moreover, equation~\eqref{eqn:weight-subset-two} holds for all set $A$ if $Y|X = Y|X_{S}$.
This shows for any set $A$: % \subseteq S$: 
\begin{equation*}
\begin{split}
\popexpB[w_A(X, Y) w_A(X', Y')] &= \E[\pi(X_A)(1-\pi(X_A')) \mid Y =0, Y' = 1]  \\
	&=  \E[\pi(X_A) \mid Y=0] \cdot \E[(1-\pi(X_A)) \mid Y=1] \\
	&\ge \E[\pi(X_S) \mid Y=0] \cdot \E[(1-\pi(X_S)) \mid Y=1] \\
	&\ge \varrho^2,
\end{split}
\end{equation*}
where the first inequality uses our previous results. One can prove analogously the bound
$\popexpW[w_A(X, Y) w_A(X', Y')] \ge \varrho^{2}$.





